Data-driven Distributed and Localized Model Predictive Control

Motivated by large-scale but computationally constrained settings, e.g., the Internet of Things, we present a novel data-driven distributed control algorithm that is synthesized directly from trajectory data. Our method, data-driven Distributed and Localized Model Predictive Control (D$^3$LMPC), builds upon the data-driven System Level Synthesis (SLS) framework, which allows one to parameterize \emph{closed-loop} system responses directly from collected open-loop trajectories. The resulting model-predictive controller can be implemented with distributed computation and only local information sharing. By imposing locality constraints on the system response, we show that the amount of data needed for our synthesis problem is independent of the size of the global system. Moreover, we show that our algorithm enjoys theoretical guarantees for recursive feasibility and asymptotic stability. Finally, we also demonstrate the optimality and scalability of our algorithm in a simulation experiment.

==> tex_files/head.tex <==
\title{Data-driven Distributed and Localized Model Predictive Control}
\author{Carmen~Amo~Alonso\thanks{Denotes equal contribution. $^1$C. Amo Alonso is with the Dept. of Computing and Mathematical Sciences, California Institute of Technology, Pasadena, CA. $^2$F. Yang is with the Dept. of Computer and Information Sciences, University of Pennsylvania, Philadelphia, PA. $^3$N. Matni is with the Dept. of Electrical and Systems Engineering, University of Pennsylvania, Philadelphia, PA. }$^{\ 1}$, Fengjun Yang$^{*2}$ and Nikolai Matni$^{3}$
\thanks{N. Matni is generously supported by NSF award CPS-2038873, NSF CAREER award ECCS-2045834, and Google Research Scholar Award.}
}
